Semantics for Locking Specifications

To prevent concurrency errors, programmers need to obey a locking discipline. Annotations that specify that discipline, such as Java's @GuardedBy, are already widely used. Unfortunately, their semantics is expressed informally and is consequently ambiguous. This article highlights such ambiguities and formalizes the semantics of @GuardedBy in two alternative ways, building on an operational semantics for a small concurrent fragment of a Java-like language. It also identifies when such annotations are actual guarantees against data races. Our work aids in understanding the annotations and supports the development of sound formal tools that verify or infer such annotations.

==> deadlock.tex <==
\subsection{Some definitions which may be useful at some point}
\begin{definition}[Deadlock freedom]
We say that an initial configuration of a program $\anglepair{T_0}{\mu_0}$
is \emph{deadlock free} if and only if for every trace 
\[ 
\anglepair{T_0}{\mu_0}\trans{}^*\anglepair{\thread{S_1}{\lockset_1}\parallel
%\thread{S_2}{\lockset_2}\parallel
\ldots\parallel \thread{S_n}{\lockset_n}\,}{\mu}
\]
there are no  $i,j\in\{1\ldots n\}$,  $i\neq j$, for which: 
\begin{itemize}
\item 
 $S_i = \record{k_i.m_i}{\synch{E_i}{C_i};C'_i}{s_i} \stsep S_i$,
 for some $k_i,m_i,C_i,E_i,C'_i,s_i$ and $S_i$, with 
  $\eval{E_i}{\mu_i}{s_i} = \langle l_i,\hat{\mu_i}\rangle$ 
\item $S_j = \record{k_j.m_j}{\synch{E_j}{C_j};C'_j}{s_j} \stsep S_j$,
 for some $k_j,m_j,C_j,E_j,C'_j,s_j$ and $S_j$, with 
  $\eval{E_j}{\mu_j}{s_j} = \langle l_j,\hat{\mu_j}\rangle$ 
\end{itemize}
 where $l_i \in \lockset_j$ and $l_j \in \lockset_i$. 
\end{definition}



==> holding.tex <==
\section{Holding}\label{sec:holding}
%
% \jt {If you mention the existence of the Holding annotation without some explanation for its need,
% the user might not know why they should be interested in it. Also, it might be worth explaining
% that Holding originally came from GuardedBy in JCIP, and it is a way to further avoid ambiguity
% in GuardedBy. The section in the Checker Framework manual entitled
% "Relationship to annotations in Java Concurrency in Practice" describes the exact reasons why
% GuardedBy was split into GuardedBy and Holding.}
We want to define, in a formal way, the meaning, for a method $k.m$, of being \emph{holding} a lock expression $E$.
Here, $E$ can be any expression not involving the special variable $\mathtt{container}$.
The intuition behind $k.m$ being $\holding{E}$ is that, whenever a thread starts the execution of $k.m$,
that thread must hold the lock on (the then current value of) $E$. Note that this means that $E$ should be evaluated
at the beginning of $k.m$, where only $\this$ is in scope, not in the scope of the callers of $k.m$.
Since, at its beginning, a thread does not hold any lock, no method called by a $\fork{}$ can ever
be holding any expression.

%This definition captures $\mathit{Holding}$ annotation just on the invocation of the method $k.m$ without considering the fact that it may be overridden.

\begin{definition}[$\mathtt{Holding}$ for Methods] Given a program and a method $k.m$, we say that
\emph{$k.m$ is $\holding{E}$} if and only if for every derivation
\[
  \anglepair{T_0}{\mu_0}\ \trans{}^*\ \anglepair{T}{\mu}\reduces{n}\anglepair{T'}{\mu'},
\]
%%\begin{itemize}
%\item
where the $n$-th thread in  $T$ is $\thread{\record{k'.m'}{C}{s}\stsep S)}{mathcal{L}}$
with $C=E'.m(\,);C'$ or $C=\fork{E'.m(\,)};C'$, 
and the $n$-th thread in $T'$ is $\thread{\record{k.m}{B}{s'}\stsep {S'}}{\mathcal{L}'}$, for some $B$, 
%\item $C=E'.m(\,);C'$ or $C=\fork{E'.m(\,)};C'$
%%\item $\eval{E'}{s}{\mu} = \anglepair{l}{\mu'}$ and  $\cls{\mu'(l)} = k'$
%\end{itemize}
%
%%either
%% $\lookup{k'.m} \not= k$ or ($C=E'.m(\,);C'$ and 
it holds that $\loc{\eval{E}{\mu'}{s'}}\in\mathcal{L}'$.\qed
\end{definition}


==> overriding.tex <==
\section{Method Overriding}\label{sec:overriding}

Now a first attempt to deal with overriding. We need to capture all the overridings for $k.m$, thus we ask for $\lookup{k'.m}\leq k$ instead of $\lookup{k'.m}= k$.

\begin{definition}[$\mathtt{Holding}$ for method invocation and overriding] Given a program and a method $m(\,)$  defined by class $k$, we say that
\emph{$m(\,)$ is $\holding{E}$} if and only if for every derivation
\[
  \anglepair{\record{\initk.\mathit{main}}{C_{\mathit{main}}}{\inits}}{\initmu}\ \trans{}^*\ \anglepair{T}{\mu}\reduces{n}\anglepair{T'}{\mu'},
\]
where the $n$-th thread in the thread pool $T$ is $(\record{k'.m'}{C}{s}\stsep S)\{\tilde{l}\}$ 
with %either 
$C=E'.m(\,);C'$ %or $C=\fork{E'.m(\,)};C'$ 
where $\eval{E'}{s}{\mu} = \anglepair{l}{\mu'}$, $\cls{\mu'(l)} = k'$ and $\lookup{k'.m}\leq k$ , then we
have \[\first{\eval{E\subst{E'}{\this}}{\mu}{s}}\in\tilde{l}\].
\end{definition}

